AVS-Mamba: Exploring Temporal and Multi-modal Mamba for Audio-Visual Segmentation

The essence of audio-visual segmentation (AVS) lies in locating and delineating sound-emitting objects within a video stream. While Transformer-based methods have shown promise, their handling of long-range dependencies struggles due to quadratic computational costs, presenting a bottleneck in complex scenarios. To overcome this limitation and facilitate complex multi-modal comprehension with linear complexity, we introduce AVS-Mamba, a selective state space model to address the AVS task. Our framework incorporates two key components for video understanding and cross-modal learning: Temporal Mamba Block for sequential video processing and Vision-to-Audio Fusion Block for advanced audio-vision integration. Building on this, we develop the Multi-scale Temporal Encoder, aimed at enhancing the learning of visual features across scales, facilitating the perception of intra- and inter-frame information. To perform multi-modal fusion, we propose the Modality Aggregation Decoder, leveraging the Vision-to-Audio Fusion Block to integrate visual features into audio features across both frame and temporal levels. Further, we adopt the Contextual Integration Pyramid to perform audio-to-vision spatial-temporal context collaboration. Through these innovative contributions, our approach achieves new state-of-the-art results on the AVSBench-object and AVSBench-semantic datasets. Our source code and model weights are available at AVS-Mamba.

==> Table/ablation_semantic.tex <==
\begin{table*}[htbp]
\begin{minipage}{0.5\textwidth}
    \centering
    \vspace{-2mm}
    \captionsetup{width=.8\textwidth}
    \caption{Overall components analysis. The outcomes demonstrate the effectiveness of proposed modules. }
    \label{Ablation study of overall components}
    \begin{tabular}{ccccc}
    \toprule
    % 这里的各个实验及模块的名称待定
         \multirow{2}{*}{Module} &\multicolumn{2}{c}{MS3}&\multicolumn{2}{c}{S4}\\
         & \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\) & \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         AVS-Mamba&  \textbf{68.6}& \textbf{78.8}\\
         $\it{w/o}$ MTE&  66.8 & \underline{77.3}\\
         $\it{w/o}$ MAD& 65.4&75.7\\
         $\it{w/o}$ CIP& \underline{67.1}&77.0\\
    \bottomrule
    \end{tabular}
    % \vspace{-3mm}
\end{minipage}
\begin{minipage}{0.5\textwidth}
    \centering
    \vspace{-2mm}
    \captionsetup{width=.8\textwidth}
    \caption{Effect of Multi-scale Temporal Encoder. Both VSS block and Temporal Mamba block are pivotal in multi-scale interactions. }
    \label{Ablation study of Multi-scale Temporal Encoder}
   \begin{tabular}{ccccc}
    \toprule
    % 这里的各个实验及模块的名称待定
         \multirow{2}{*}{Components} &\multicolumn{2}{c}{MS3}&\multicolumn{2}{c}{S4}\\
         & \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)& \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         $\it{w/o}$ Encoder&  66.8& 77.3\\
         $\it{w/o}$ VSS Block&  \underline{68.1}& \underline{77.4}\\
         $\it{w/o}$ Temporal Mamba& 67.6&77.2\\
         Ours& \textbf{68.6}&\textbf{78.8}\\
    \bottomrule
    \end{tabular}
    % \vspace{-3mm}
\end{minipage}
% \begin{minipage}{0.3\textwidth}
%     \centering
%     \begin{tabular}{cccc}
%     \toprule
%     % 这里的各个实验及模块的名称待定
%          \multicolumn{2}{c}{Num. of Scan Sequences}& \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
%          \midrule
%          \multicolumn{2}{c}{2}&  67.6& \underline{77.3}\\
%          \multicolumn{2}{c}{4}&  67.8& 77.0\\
%          \multicolumn{2}{c}{6}& \textbf{68.7}&\underline{77.3}\\
%          \multicolumn{2}{c}{8}& \underline{68.6}&\textbf{78.8}\\
%     \bottomrule
%     \end{tabular}
%     \captionsetup{width=.9\textwidth}
%     \caption{Ablation study of scan order}
%     \label{Ablation study of scan order}
% \end{minipage}
\end{table*}

==> Table/ablation_study1.tex <==
\begin{table*}[htbp]
\begin{minipage}{0.35\textwidth}
    \centering
    \vspace{-2mm}
     \captionsetup{width=.9\textwidth}
    \caption{Modality Aggregation Decoder Analysis. The effects of executing frame- and temporal-level cross-modal fusion outperforms the methods engaging in either of them. }
    \label{Ablation study of Modality Aggregation Decoder}
    \begin{tabular}{ccccc}
    \toprule
    % 这里的各个实验及模块的名称待定
         \multirow{2}{*}{Components}& \multicolumn{2}{c}{MS3} & \multicolumn{2}{c}{S4}\\
         &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         $\it{w/o}$ Decoder &  65.4& 75.7&  & \\
         $\it{w/o}$ Frame-level &  \underline{67.0}& \underline{77.1}& & \\
         $\it{w/o}$ Temporal-level & 66.6&76.8&&\\
         Ours & \textbf{68.6}&\textbf{78.8}&&\\
    \bottomrule
    \end{tabular}
    % \vspace{-6mm}
\end{minipage}
\begin{minipage}{0.35\textwidth}
    \centering
    \vspace{-2mm}
    \captionsetup{width=.9\textwidth}
    \caption{Ablation study of Contextual Integration Pyramid. Omitting either the Temporal Mamba or the A2V Fusion results in diminished performance.}
    \label{Ablation study of Contextual Integration Pyramid}
    \begin{tabular}{ccccc}
    \toprule
          \multirow{2}{*}{Components}& \multicolumn{2}{c}{MS3} & \multicolumn{2}{c}{S4}\\
          & \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)& \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         % 这里的各个实验及模块的名称待定
         $\it{w/o}$ CIP&  67.1& 77.0&&\\
         $\it{w/o}$ Temporal Mamba&  67.9& 76.8&&\\
         $\it{w/o}$ A2V Fusion & \underline{68.5}&\underline{78.1}&&\\
         Ours & \textbf{68.6}&\textbf{78.8}&&\\
    \bottomrule
    \end{tabular}
    % \vspace{-6mm}
\end{minipage}
\begin{minipage}{0.25\textwidth}
    \centering
    \vspace{-2mm}
    \captionsetup{width=.8\textwidth}
    \caption{Impact of scan order in Temporal Mamba. Utilizing eight scan sequences achieves optimal results.}
    \label{Ablation study of scan order}
    \begin{tabular}{ccccc}
    \toprule
    % 这里的各个实验及模块的名称待定
        \multirow{2}{*}{Num.}& \multicolumn{2}{c}{MS3} & \multicolumn{2}{c}{S4}\\
         & \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)& \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         2&  67.6& \underline{77.3}&&\\
         4&  67.8& 77.0&&\\
         6& \textbf{68.7}&\underline{77.3}&&\\
         8 (Ours)& \underline{68.6}&\textbf{78.8}&&\\
    \bottomrule
    \end{tabular}
    % \vspace{-6mm}
\end{minipage}
\end{table*}

==> Table/algorithm.tex <==

% \documentclass[11pt]{ctexart}
% \usepackage[top=2cm, bottom=2cm, left=2.5cm, right=2.5cm]{geometry} %定义页边距
% \usepackage{algorithm}
% \usepackage{algorithmicx}
% \usepackage{algpseudocode}
% \usepackage{amsmath} %数学公式
% \floatname{algorithm}{Algorithm} %算法
% \renewcommand{\algorithmicrequire}{\textbf{Input:}} %输入
% \renewcommand{\algorithmicensure}{\textbf{Output:}} %输出

% \begin{document}
% \definecolor{lightskyblue}{RGB}{135, 206, 250}
\begin{algorithm}
\caption{Contextual Integration Pyramid}
\label{Contextual Integration Pyramid}
\vspace{-4mm}
\begin{algorithmic}[1]
\Require $\bar{F}_{a}: \textcolor[RGB]{61,154,64}{(B,T,C)},\{F^{i}_{v'}\}^{4}_{i=2},F^{1}_{v}:\textcolor[RGB]{61,154,64}{(B,T,h_{i},w_{i},C)}$
\Ensure $\mathcal{F}:\textcolor[RGB]{61,154,64}{(B,T,h_{1},w_{1},C)}$
\State $\{\bar{F}^{i}_{v}\}^{4}_{i=1}=\{F^{1}_{v},F^{2}_{v'},F^{3}_{v'},F^{4}_{v'}\}$
\For{$i = 4 \to 1$}
    \State $\mathbf{\tilde{F}^{i}_{v}} : \textcolor[RGB]{61,154,64}{(B, T, h_{i}, w_{i}, C)} \leftarrow Temporal Mamba(\bar{F}^{i}_{v})$   
    \State \textbf{Pre-Processing}
    \State $\mathbf{\tilde{F}^{i}_{v'}} : \textcolor[RGB]{61,154,64}{(B,T,h_{i},w_{i},C)} \leftarrow DWConv2d(Linear1(Norm(\tilde{F}^{i}_{v})))$
    \State $\mathbf{F^{i}_{z}} : \textcolor[RGB]{61,154,64}{(B, T, h_{i}, w_{i}, C)} \leftarrow SiLU(Linear2(Norm(\tilde{F}^{i}_{v})))$
    \State $\mathbf{\tilde{F}_{a}}:\textcolor[RGB]{61,154,64}{(B, T, C)} \leftarrow Conv1d(Linear3(Norm1(\bar{F}_{a})))$
    \State \textbf{Serialization+Combination}
    \State $\mathbf{F^{i}_{sv}}:\textcolor[RGB]{61,154,64}{(B, 2, Th_{i}w_{i}, C)} \leftarrow Concat(F_{TWH}(\tilde{F}^{i}_{v'}),F_{THW}(\tilde{F}^{i}_{v'}))$
    \State $\mathbf{\tilde{F}_{a'}}:\textcolor[RGB]{61,154,64}{(B, 4, T, C)} \leftarrow Concat(\tilde{F}_{a}, Reverse(\tilde{F}_{a}))$
    \State $\mathbf{\tilde{F}^{i}_{sv}} : \textcolor[RGB]{61,154,64}{(B, 4, Th_{i}w_{i}, C)} \leftarrow Concat(F^{i}_{sv}, Reverse(F^{i}_{sv}))$
    \State $\mathbf{\tilde{F}^{i}_{av}} : \textcolor[RGB]{61,154,64}{(B, 4, T + Th_{i}w_{i}, C)}
    \leftarrow Concat(\tilde{F}_{a'}, \tilde{F}^{i}_{sv})$
    \State \textbf{SSM + Post-Processing}
    \State $\mathbf{\hat{F}^{i}_{v'}} : \textcolor[RGB]{61,154,64}{(B, T, h_{i}, w_{i}, C)} 
    \leftarrow \sum^{4}_{k=1}{Partition_{k}(SSM_{k}(\tilde{F}^{i}_{av}[:,k]))}$
    \State $\mathbf{\mathcal{F}^{i}_{v}} : \textcolor[RGB]{61,154,64}{(B, T, h_{i}, w_{i}, C)} \leftarrow Linear4(Norm2(\hat{F}^{i}_{v'})\times{F^{i}_{z}})+\tilde{F}^{i}_{v}$
\EndFor
\State $\mathcal{F} \leftarrow Up_{\times{8}}(\mathcal{F}^{4}_{v})+Up_{\times{4}}(\mathcal{F}^{3}_{v})+Up_{\times{2}}(\mathcal{F}^{2}_{v})+\mathcal{F}^{1}_{v}$ 
\end{algorithmic}
\end{algorithm}
% \vspace{-2mm}
% \end{document}

